Rewards Encoding Environment Dynamics Improves Preference-based Reinforcement Learning

Preference-based reinforcement learning (RL) algorithms help avoid the pitfalls of hand-crafted reward functions by distilling them from human preference feedback, but they remain impractical due to the burdensome number of labels required from the human, even for relatively simple tasks. In this work, we demonstrate that encoding environment dynamics in the reward function (REED) dramatically reduces the number of preference labels required in state-of-the-art preference-based RL frameworks. We hypothesize that REED-based methods better partition the state-action space and facilitate generalization to state-action pairs not included in the preference dataset. REED iterates between encoding environment dynamics in a state-action representation via a self-supervised temporal consistency task, and bootstrapping the preference-based reward function from the state-action representation. Whereas prior approaches train only on the preference-labelled trajectory pairs, REED exposes the state-action representation to all transitions experienced during policy training. We explore the benefits of REED within the PrefPPO [1] and PEBBLE [2] preference learning frameworks and demonstrate improvements across experimental conditions to both the speed of policy learning and the final policy performance. For example, on quadruped-walk and walker-walk with 50 preference labels, REED-based reward functions recover 83% and 66% of ground truth reward policy performance and without REED only 38\% and 21\% are recovered. For some domains, REED-based reward functions result in policies that outperform policies trained on the ground truth reward.

==> complete_perf_ratios_table.tex <==
\begin{landscape}
\begin{center}
\begin{scriptsize}
\begin{sc}
\begin{longtable}{lll @{\hspace{1cm}} cccccc @{\hspace{1cm}} c}
\caption{Ratio of policy performance on learned versus ground truth rewards for \textbf{walker-walk}, \textbf{cheetah-run}, \textbf{quadruped-walk}, \textbf{sweep into}, and \textbf{button press} across preference learning methods, labelling methods and feedback amounts (with disagreement sampling). The results are reported as means (standard deviations) over 10 random seeds.} \label{app_tab:all_normalized_returns} \\

% First header
\toprule
 & Feedback & Method & Oracle & Mistake & Equal & Skip & Myopic & Noisy & Mean \\
\midrule
\endfirsthead

% Normal header
\multicolumn{10}{c}%
{\textbf{\bfseries \tablename\ \thetable{}} -- \textit{continued from previous page}}\\
\toprule
 & Feedback & Method & Oracle & Mistake & Equal & Skip & Myopic & Noisy & Mean \\
\midrule
\endhead

% Normal footer
\\
\multicolumn{10}{r}{\textit{Continues on next page...}} \\ 
\bottomrule 
\endfoot

% Last footer
\bottomrule
\endlastfoot

%% WALKER-STAND RESULTS [NOT INCLUDED IN FINAL VERSION]
% \multicolumn{10}{c}{Walker-stand}  \\
% \midrule

% & \multirow{7}{*}{1k} & PEBBLE & 0.9 (0.16) & 0.84 (0.19) & 0.93 (0.15) & 0.91 (0.16) & 0.83 (0.15) & 0.9 (0.16) & 0.88 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.93 (0.16) & 0.86 (0.19) & 0.93 (0.15) & 0.92 (0.16) & 0.88 (0.19) & 0.91 (0.17) & 0.91 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.95 (0.14) & 0.84 (0.16) & 0.95 (0.12) & 0.95 (0.14) & 0.89 (0.18) & 0.93 (0.16) & 0.92 \\ 
%  \\
%  & & PrefPPO & 0.95 (0.015) & 0.89 (0.025) & 0.97 (0.015) & 0.97 (0.021) & 0.93 (0.018) & 0.94 (0.012) & 0.94 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.96 (0.017) & 0.89 (0.013) & 0.99 (0.016) & 0.95 (0.021) & 0.91 (0.021) & 0.97 (0.014) & 0.95 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.97 (0.023) & 0.92 (0.016) & 0.96 (0.02) & 0.97 (0.025) & 0.91 (0.019) & 0.95 (0.019) & 0.95 \\ 
%  \cmidrule{2-10}
% & \multirow{7}{*}{500} & PEBBLE & 0.82 (0.19) & 0.65 (0.14) & 0.86 (0.18) & 0.83 (0.19) & 0.76 (0.15) & 0.78 (0.16) & 0.79 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.9 (0.2) & 0.8 (0.19) & 0.91 (0.18) & 0.9 (0.19) & 0.87 (0.2) & 0.89 (0.2) & 0.88 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.93 (0.16) & 0.87 (0.19) & 0.94 (0.16) & 0.92 (0.18) & 0.88 (0.18) & 0.92 (0.18) & 0.91 \\ 
%  \\
%  & & PrefPPO & 0.93 (0.0098) & 0.87 (0.014) & 0.94 (0.015) & 0.92 (0.0091) & 0.87 (0.013) & 0.9 (0.011) & 0.91 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.9 (0.019) & 0.88 (0.019) & 0.94 (0.022) & 0.91 (0.02) & 0.88 (0.022) & 0.91 (0.015) & 0.90 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.94 (0.019) & 0.82 (0.03) & 0.94 (0.013) & 0.91 (0.013) & 0.85 (0.025) & 0.93 (0.021) & 0.90 \\ 
%  \cmidrule{2-10}
% & \multirow{7}{*}{200} & PEBBLE & 0.64 (0.14) & 0.53 (0.11) & 0.64 (0.13) & 0.69 (0.17) & 0.47 (0.095) & 0.65 (0.16) & 0.60 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.85 (0.23) & 0.72 (0.2) & 0.85 (0.23) & 0.85 (0.23) & 0.74 (0.21) & 0.81 (0.24) & 0.80 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.87 (0.21) & 0.73 (0.15) & 0.89 (0.2) & 0.87 (0.21) & 0.75 (0.18) & 0.86 (0.21) & 0.83 \\ 
%  \\
%  & & PrefPPO & 0.84 (0.024) & 0.83 (0.017) & 0.86 (0.018) & 0.85 (0.018) & 0.79 (0.028) & 0.84 (0.018) & 0.84 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.83 (0.032) & 0.78 (0.033) & 0.85 (0.032) & 0.8 (0.028) & 0.76 (0.031) & 0.78 (0.029) & 0.80 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.8 (0.031) & 0.83 (0.017) & 0.84 (0.018) & 0.84 (0.022) & 0.81 (0.021) & 0.84 (0.022) & 0.83 \\
%  \cmidrule{2-10}
% & \multirow{7}{*}{100} & PEBBLE & 0.48 (0.089) & 0.39 (0.079) & 0.58 (0.13) & 0.45 (0.082) & 0.32 (0.06) & 0.41 (0.072) & 0.44 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.74 (0.22) & 0.68 (0.19) & 0.73 (0.18) & 0.8 (0.24) & 0.62 (0.16) & 0.78 (0.24) & 0.73 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.83 (0.21) & 0.71 (0.18) & 0.79 (0.2) & 0.86 (0.22) & 0.62 (0.15) & 0.84 (0.23) & 0.78 \\ 
% \\
%  & & PrefPPO & 0.75 (0.032) & 0.69 (0.041) & 0.79 (0.024) & 0.73 (0.038) & 0.61 (0.067) & 0.7 (0.048) & 0.71 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.74 (0.029) & 0.7 (0.045) & 0.81 (0.028) & 0.81 (0.034) & 0.71 (0.04) & 0.74 (0.042) & 0.75 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.8 (0.03) & 0.67 (0.046) & 0.79 (0.035) & 0.75 (0.036) & 0.69 (0.035) & 0.79 (0.028) & 0.75 \\ 
%  \cmidrule{2-10}
% & \multirow{7}{*}{50} & PEBBLE & 0.3 (0.064) & 0.28 (0.054) & 0.39 (0.081) & 0.3 (0.057) & 0.29 (0.067) & 0.36 (0.058) & 0.32 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.67 (0.19) & 0.57 (0.13) & 0.72 (0.22) & 0.69 (0.22) & 0.54 (0.15) & 0.63 (0.19) & 0.64 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.68 (0.18) & 0.55 (0.13) & 0.78 (0.21) & 0.66 (0.18) & 0.53 (0.12) & 0.71 (0.19) & 0.65 \\ 
%  \\
%  &  & PrefPPO & 0.56 (0.071) & 0.57 (0.084) & 0.67 (0.047) & 0.63 (0.071) & 0.49 (0.096) & 0.66 (0.061) & 0.60 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.7 (0.042) & 0.54 (0.087) & 0.7 (0.046) & 0.55 (0.077) & 0.62 (0.06) & 0.62 (0.057) & 0.62 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.67 (0.053) & 0.62 (0.061) & 0.7 (0.043) & 0.71 (0.037) & 0.55 (0.09) & 0.61 (0.068) & 0.64 \\
%  \midrule

 %% WALKER-WALK RESULTS
\multicolumn{10}{c}{Walker-walk}  \\
\midrule
 
 & \multirow{7}{*}{1k} & PEBBLE & 0.85 (0.17) & 0.76 (0.21) & 0.88 (0.16) & 0.85 (0.17) & 0.79 (0.18) & 0.81 (0.18) & 0.83 \\ 
 & & \hspace{4 mm}+SimSiam  & 0.9 (0.16) & 0.77 (0.2) & 0.91 (0.12) & 0.89 (0.16) & 0.8 (0.17) & 0.88 (0.17) & 0.86 \\ 
 & & \hspace{4 mm}+Contr.  & 0.9 (0.16) & 0.77 (0.2) & 0.91 (0.12) & 0.89 (0.16) & 0.8 (0.17) & 0.88 (0.17) & 0.86 \\ 
 \\
 & & PrefPPO & 1.0 (0.034) & 0.92 (0.056) & 1.0 (0.029) & 1.0 (0.031) & 1.0 (0.044) & 0.96 (0.056) & 0.99 \\ 
 & & \hspace{4 mm}+SimSiam & 1.1 (0.025) & 0.92 (0.05) & 1.0 (0.031) & 1.0 (0.02) & 0.99 (0.035) & 0.96 (0.046) & 1.00 \\ 
 & & \hspace{4 mm}+Contr. & 1.0 (0.029) & 0.93 (0.043) & 1.1 (0.021) & 1.0 (0.028) & 0.98 (0.033) & 0.95 (0.045) & 1.00 \\
 \cmidrule{2-10}
& \multirow{7}{*}{500} & PEBBLE & 0.74 (0.18) & 0.61 (0.17) & 0.84 (0.19) & 0.75 (0.19) & 0.67 (0.19) & 0.69 (0.19) & 0.72 \\
 & & \hspace{4 mm}+SimSiam & 0.86 (0.2) & 0.71 (0.2) & 0.87 (0.2) & 0.87 (0.2) & 0.82 (0.22) & 0.84 (0.2) & 0.83 \\ 
 & & \hspace{4 mm}+Contr. & 0.9 (0.17) & 0.81 (0.19) & 0.9 (0.14) & 0.9 (0.17) & 0.88 (0.16) & 0.88 (0.18) & 0.88 \\ 
 \\
 & & PrefPPO & 0.95 (0.052) & 0.83 (0.087) & 0.95 (0.044) & 0.96 (0.058) & 0.89 (0.076) & 0.88 (0.069) & 0.91 \\
 & & \hspace{4 mm}+SimSiam & 0.88 (0.074) & 0.81 (0.084) & 0.98 (0.025) & 0.95 (0.027) & 0.9 (0.073) & 0.9 (0.069) & 0.90 \\ 
 & & \hspace{4 mm}+Contr. & 0.93 (0.061) & 0.85 (0.077) & 0.95 (0.046) & 0.92 (0.059) & 0.82 (0.085) & 0.77 (0.098) & 0.88 \\
 \cmidrule{2-10}
& \multirow{7}{*}{200} & PEBBLE & 0.52 (0.17) & 0.46 (0.15) & 0.67 (0.2) & 0.54 (0.15) & 0.46 (0.13) & 0.45 (0.14) & 0.52 \\ 
 & & \hspace{4 mm}+SimSiam & 0.74 (0.2) & 0.65 (0.21) & 0.79 (0.22) & 0.74 (0.19) & 0.64 (0.21) & 0.8 (0.25) & 0.73 \\ 
 & & \hspace{4 mm}+Contr. & 0.84 (0.2) & 0.69 (0.2) & 0.84 (0.18) & 0.84 (0.2) & 0.75 (0.19) & 0.84 (0.21) & 0.80 \\ 
 \\
 & & PrefPPO & 0.93 (0.058) & 0.83 (0.076) & 0.93 (0.027) & 0.88 (0.045) & 0.87 (0.079) & 0.82 (0.06) & 0.88 \\ 
 & & \hspace{4 mm}+SimSiam & 0.78 (0.087) & 0.68 (0.11) & 0.81 (0.062) & 0.77 (0.081) & 0.77 (0.077) & 0.78 (0.053) & 0.77 \\ 
 & & \hspace{4 mm}+Contr. & 0.81 (0.088) & 0.81 (0.079) & 0.86 (0.044) & 0.85 (0.055) & 0.76 (0.13) & 0.74 (0.1) & 0.80 \\ 
 \cmidrule{2-10}
& \multirow{7}{*}{100} & PEBBLE & 0.34 (0.11) & 0.31 (0.11) & 0.37 (0.1) & 0.37 (0.12) & 0.29 (0.085) & 0.41 (0.13) & 0.35 \\
 & & \hspace{4 mm}+SimSiam & 0.68 (0.23) & 0.57 (0.2) & 0.72 (0.25) & 0.67 (0.23) & 0.61 (0.19) & 0.66 (0.24) & 0.65 \\
 & & \hspace{4 mm}+Contr. & 0.78 (0.21) & 0.69 (0.22) & 0.74 (0.22) & 0.74 (0.19) & 0.68 (0.19) & 0.74 (0.22) & 0.73 \\ 
 \\
 & & PrefPPO & 0.68 (0.08) & 0.59 (0.093) & 0.73 (0.065) & 0.73 (0.065) & 0.58 (0.11) & 0.68 (0.072) & 0.67 \\
 & & \hspace{4 mm}+SimSiam & 0.67 (0.08) & 0.63 (0.11) & 0.71 (0.075) & 0.71 (0.084) & 0.63 (0.099) & 0.63 (0.094) & 0.66 \\ 
 & & \hspace{4 mm}+Contr. & 0.72 (0.084) & 0.49 (0.14) & 0.71 (0.063) & 0.65 (0.091) & 0.64 (0.1) & 0.58 (0.13) & 0.63 \\ 
 \cmidrule{2-10}
& \multirow{7}{*}{50} & PEBBLE & 0.21 (0.1) & 0.22 (0.12) & 0.22 (0.12) & 0.23 (0.14) & 0.21 (0.11) & 0.18 (0.11) & 0.21 \\ 
 & & \hspace{4 mm}+SimSiam & 0.66 (0.24) & 0.44 (0.13) & 0.6 (0.21) & 0.64 (0.24) & 0.44 (0.12) & 0.48 (0.15) & 0.54 \\
 & & \hspace{4 mm}+Contr. & 0.62 (0.22) & 0.44 (0.11) & 0.72 (0.22) & 0.62 (0.22) & 0.54 (0.16) & 0.54 (0.17) & 0.58 \\ 
 \\
 & & PrefPPO & 0.51 (0.13) & 0.41 (0.18) & 0.57 (0.12) & 0.59 (0.11) & 0.51 (0.14) & 0.51 (0.14) & 0.52 \\ 
 & & \hspace{4 mm}+SimSiam & 0.58 (0.13) & 0.41 (0.17) & 0.6 (0.13) & 0.56 (0.13) & 0.58 (0.12) & 0.48 (0.13) & 0.54 \\ 
 & & \hspace{4 mm}+Contr. & 0.58 (0.12) & 0.54 (0.15) & 0.62 (0.12) & 0.63 (0.11) & 0.5 (0.13) & 0.57 (0.12) & 0.57 \\ 
\midrule


%% WALKER-RUN RESULTS [[NOT INCLUDED IN FINAL VERSION]]
% \multicolumn{10}{c}{Walker-run}  \\
% \midrule


%   & \multirow{7}{*}{1k} & PEBBLE & 0.71 (0.25) & 0.57 (0.2) & 0.76 (0.23) & 0.7 (0.26) & 0.58 (0.25) & 0.58 (0.19) & 0.65 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.78 (0.2) & 0.53 (0.16) & 0.8 (0.19) & 0.78 (0.2) & 0.57 (0.15) & 0.62 (0.17) & 0.68 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.8 (0.16) & 0.69 (0.17) & 0.82 (0.17) & 0.83 (0.19) & 0.7 (0.18) & 0.69 (0.16) & 0.76 \\ 
%  & & PrefPPO & 0.99 (0.012) & 0.92 (0.023) & 1.0 (0.012) & 0.99 (0.03) & 0.96 (0.047) & 0.86 (0.048) & 0.95 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.0 (0.0079) & 0.92 (0.012) & 0.97 (0.021) & 0.96 (0.016) & 0.89 (0.069) & 0.88 (0.038) & 0.94 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.98 (0.016) & 0.9 (0.036) & 0.99 (0.018) & 1.0 (0.0099) & 0.87 (0.056) & 0.88 (0.045) & 0.94 \\ 
%  \cmidrule{2-10}
% & \multirow{7}{*}{500} & PEBBLE & 0.59 (0.24) & 0.4 (0.22) & 0.62 (0.27) & 0.57 (0.24) & 0.44 (0.21) & 0.46 (0.2) & 0.51 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.72 (0.21) & 0.59 (0.2) & 0.71 (0.21) & 0.72 (0.21) & 0.59 (0.18) & 0.53 (0.16) & 0.65 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.75 (0.19) & 0.64 (0.17) & 0.79 (0.21) & 0.75 (0.19) & 0.66 (0.19) & 0.57 (0.17) & 0.69 \\ 
%  & & PrefPPO & 0.95 (0.035) & 0.93 (0.03) & 0.93 (0.028) & 0.91 (0.028) & 0.88 (0.07) & 0.85 (0.044) & 0.91 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.93 (0.015) & 0.89 (0.036) & 0.96 (0.01) & 0.92 (0.02) & 0.78 (0.081) & 0.86 (0.038) & 0.89 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.93 (0.039) & 0.83 (0.054) & 0.95 (0.016) & 0.96 (0.018) & 0.86 (0.061) & 0.82 (0.047) & 0.89 \\
%  \cmidrule{2-10}
% & \multirow{7}{*}{200} & PEBBLE & 0.44 (0.24) & 0.31 (0.2) & 0.45 (0.22) & 0.4 (0.22) & 0.32 (0.21) & 0.23 (0.16) & 0.36 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.62 (0.22) & 0.46 (0.17) & 0.61 (0.22) & 0.63 (0.23) & 0.42 (0.15) & 0.5 (0.2) & 0.54 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.68 (0.19) & 0.43 (0.14) & 0.68 (0.2) & 0.67 (0.19) & 0.6 (0.17) & 0.59 (0.18) & 0.61 \\ 
%  & & PrefPPO & 0.83 (0.033) & 0.8 (0.056) & 0.87 (0.037) & 0.85 (0.027) & 0.79 (0.058) & 0.65 (0.08) & 0.80 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.87 (0.031) & 0.81 (0.04) & 0.88 (0.021) & 0.85 (0.028) & 0.81 (0.048) & 0.74 (0.045) & 0.83 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.82 (0.032) & 0.81 (0.045) & 0.87 (0.031) & 0.85 (0.032) & 0.81 (0.04) & 0.73 (0.074) & 0.81 \\ 
%  \cmidrule{2-10}
% & \multirow{7}{*}{100} & PEBBLE & 0.25 (0.23) & 0.23 (0.26) & 0.31 (0.2) & 0.27 (0.24) & 0.18 (0.2) & 0.22 (0.22) & 0.24 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.47 (0.21) & 0.43 (0.18) & 0.54 (0.23) & 0.47 (0.21) & 0.37 (0.18) & 0.37 (0.17) & 0.44 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.61 (0.2) & 0.43 (0.15) & 0.62 (0.21) & 0.6 (0.21) & 0.39 (0.13) & 0.46 (0.19) & 0.52 \\ 
%  & & PrefPPO & 0.73 (0.045) & 0.62 (0.076) & 0.8 (0.028) & 0.73 (0.043) & 0.62 (0.078) & 0.61 (0.096) & 0.69 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.74 (0.04) & 0.6 (0.078) & 0.76 (0.036) & 0.79 (0.031) & 0.7 (0.049) & 0.66 (0.069) & 0.71 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.77 (0.039) & 0.7 (0.055) & 0.82 (0.027) & 0.72 (0.066) & 0.64 (0.061) & 0.68 (0.065) & 0.72 \\
%  \cmidrule{2-10}
% & \multirow{7}{*}{50} & PEBBLE & 0.18 (0.22) & 0.18 (0.23) & 0.2 (0.23) & 0.18 (0.22) & 0.16 (0.21) & 0.14 (0.19) & 0.17 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.42 (0.18) & 0.27 (0.14) & 0.42 (0.18) & 0.42 (0.18) & 0.25 (0.15) & 0.19 (0.14) & 0.33 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.44 (0.17) & 0.35 (0.13) & 0.47 (0.17) & 0.45 (0.17) & 0.34 (0.13) & 0.32 (0.14) & 0.40 \\ 
%  & & PrefPPO & 0.62 (0.072) & 0.55 (0.11) & 0.69 (0.07) & 0.64 (0.089) & 0.58 (0.1) & 0.56 (0.11) & 0.61 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.6 (0.082) & 0.58 (0.097) & 0.67 (0.058) & 0.78 (0.042) & 0.51 (0.12) & 0.48 (0.12) & 0.60 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.67 (0.049) & 0.59 (0.083) & 0.72 (0.045) & 0.74 (0.042) & 0.6 (0.085) & 0.54 (0.095) & 0.64 \\
%  \midrule

%% CHEETAH-RUN RESULTS 
\multicolumn{10}{c}{Cheetah-run}  \\
\midrule
 
 & \multirow{7}{*}{1k} & PEBBLE & 0.87 (0.18) & 0.82 (0.18) & 0.91 (0.2) & 0.89 (0.17) & 0.87 (0.16) & 0.82 (0.18) & 0.86 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.93 (0.2) & 0.83 (0.18) & 0.88 (0.14) & 0.92 (0.16) & 1.0 (0.18) & 0.86 (0.21) & 0.90 \\ 
 &  & \hspace{4 mm}+Contr. & 0.9 (0.17) & 0.84 (0.18) & 0.89 (0.17) & 0.96 (0.17) & 1.0 (0.21) & 0.85 (0.13) & 0.91 \\ 
 \\
 & & PrefPPO & 0.71 (0.064) & 0.72 (0.086) & 0.76 (0.069) & 0.71 (0.076) & 0.75 (0.066) & 0.69 (0.093) & 0.72 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.67 (0.054) & 0.7 (0.076) & 0.75 (0.08) & 0.66 (0.064) & 0.79 (0.084) & 0.65 (0.081) & 0.70 \\ 
 &  & \hspace{4 mm}+Contr. & 0.7 (0.069) & 0.8 (0.11) & 0.72 (0.07) & 0.71 (0.065) & 0.78 (0.089) & 0.65 (0.083) & 0.73 \\ 
 \cmidrule{2-10}
& \multirow{7}{*}{500} & PEBBLE & 0.86 (0.14) & 0.84 (0.18) & 0.86 (0.19) & 0.71 (0.16) & 0.79 (0.16) & 0.71 (0.15) & 0.79 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.88 (0.22) & 0.83 (0.18) & 0.93 (0.15) & 0.76 (0.15) & 0.85 (0.14) & 0.8 (0.19) & 0.84 \\ 
 &  & \hspace{4 mm}+Contr. & 0.94 (0.21) & 0.72 (0.14) & 0.9 (0.21) & 0.89 (0.18) & 0.93 (0.18) & 0.82 (0.16) & 0.87 \\ 
 \\
 & & PrefPPO & 0.62 (0.043) & 0.63 (0.047) & 0.77 (0.089) & 0.66 (0.06) & 0.66 (0.04) & 0.72 (0.09) & 0.67 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.67 (0.062) & 0.74 (0.14) & 0.7 (0.072) & 0.63 (0.069) & 0.67 (0.076) & 0.68 (0.081) & 0.68 \\ 
 &  & \hspace{4 mm}+Contr. & 0.66 (0.062) & 0.61 (0.072) & 0.73 (0.082) & 0.69 (0.065) & 0.61 (0.047) & 0.67 (0.073) & 0.66 \\ 
 \cmidrule{2-10}
& \multirow{7}{*}{200} & PEBBLE & 0.71 (0.23) & 0.62 (0.22) & 0.71 (0.24) & 0.57 (0.2) & 0.75 (0.18) & 0.6 (0.22) & 0.66 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.77 (0.28) & 0.61 (0.19) & 0.77 (0.22) & 0.79 (0.25) & 0.76 (0.25) & 0.65 (0.27) & 0.72 \\ 
 &  & \hspace{4 mm}+Contr. & 0.73 (0.22) & 0.67 (0.21) & 0.83 (0.25) & 0.8 (0.24) & 0.83 (0.19) & 0.76 (0.23) & 0.77 \\ 
 \\
 & & PrefPPO & 0.57 (0.042) & 0.73 (0.13) & 0.66 (0.059) & 0.54 (0.052) & 0.64 (0.073) & 0.56 (0.099) & 0.62 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.53 (0.066) & 0.52 (0.047) & 0.66 (0.066) & 0.53 (0.049) & 0.55 (0.054) & 0.57 (0.085) & 0.56 \\ 
 &  & \hspace{4 mm}+Contr. & 0.62 (0.071) & 0.49 (0.046) & 0.61 (0.06) & 0.63 (0.1) & 0.56 (0.062) & 0.58 (0.048) & 0.58 \\ 
 \cmidrule{2-10}
& \multirow{7}{*}{100} & PEBBLE & 0.4 (0.14) & 0.4 (0.13) & 0.61 (0.22) & 0.47 (0.2) & 0.55 (0.21) & 0.42 (0.14) & 0.48 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.69 (0.26) & 0.59 (0.22) & 0.79 (0.28) & 0.65 (0.29) & 0.67 (0.26) & 0.53 (0.21) & 0.65 \\ 
 &  & \hspace{4 mm}+Contr. & 0.64 (0.28) & 0.65 (0.21) & 0.78 (0.21) & 0.7 (0.29) & 0.81 (0.26) & 0.72 (0.25) & 0.72 \\ 
 \\
 & & PrefPPO & 0.46 (0.036) & 0.51 (0.061) & 0.58 (0.051) & 0.58 (0.054) & 0.6 (0.047) & 0.59 (0.054) & 0.55 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.49 (0.036) & 0.47 (0.088) & 0.49 (0.046) & 0.49 (0.038) & 0.52 (0.04) & 0.52 (0.081) & 0.50 \\ 
 &  & \hspace{4 mm}+Contr. & 0.54 (0.037) & 0.51 (0.06) & 0.59 (0.085) & 0.5 (0.059) & 0.59 (0.061) & 0.45 (0.039) & 0.53 \\ 
 \cmidrule{2-10}
& \multirow{7}{*}{50} & PEBBLE & 0.35 (0.11) & 0.26 (0.098) & 0.39 (0.14) & 0.39 (0.12) & 0.4 (0.15) & 0.24 (0.089) & 0.34 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.63 (0.23) & 0.59 (0.27) & 0.69 (0.25) & 0.62 (0.23) & 0.68 (0.31) & 0.46 (0.22) & 0.61 \\ 
 &  & \hspace{4 mm}+Contr. & 0.7 (0.28) & 0.51 (0.21) & 0.72 (0.28) & 0.53 (0.2) & 0.66 (0.28) & 0.66 (0.28) & 0.63 \\ 
 \\
 & & PrefPPO & 0.5 (0.066) & 0.49 (0.07) & 0.44 (0.076) & 0.4 (0.038) & 0.34 (0.062) & 0.3 (0.066) & 0.41 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.44 (0.041) & 0.38 (0.039) & 0.44 (0.082) & 0.3 (0.063) & 0.44 (0.085) & 0.47 (0.11) & 0.41 \\ 
 &  & \hspace{4 mm}+Contr. & 0.47 (0.051) & 0.42 (0.039) & 0.47 (0.093) & 0.43 (0.038) & 0.46 (0.039) & 0.31 (0.061) & 0.43 \\ 
\midrule

%% QUADRUPED-WALK RESULTS
\multicolumn{10}{c}{Quadruped-walk}  \\
\midrule
 & \multirow{2}{*}{2k} & PEBBLE & 0.94 (0.15) & 0.55 (0.19) & 1.1 (0.26) & 1.0 (0.16) & 0.93 (0.13) & 0.56 (0.19) & 0.86 \\ 
 &  & \hspace{4 mm}+SimSiam & 1.3 (0.31) & 0.47 (0.19) & 1.4 (0.37) & 1.3 (0.26) & 1.2 (0.18) & 0.96 (0.15) & 1.09 \\ 
 & \multirow{5}{*}{2k} & \hspace{4 mm}+Contr. & 1.3 (0.25) & 0.7 (0.16) & 1.2 (0.24) & 1.3 (0.29) & 1.3 (0.28) & 1.0 (0.16) & 1.13 \\ 
 \\
 & & PrefPPO & 1.1 (0.18) & 0.89 (0.18) & 1.2 (0.22) & 1.2 (0.17) & 1.0 (0.25) & 1.1 (0.18) & 1.07 \\ 
 &  & \hspace{4 mm}+SimSiam & 1.1 (0.22) & 1.0 (0.2) & 1.2 (0.23) & 1.1 (0.24) & 1.1 (0.26) & 0.91 (0.1) & 1.06 \\ 
 & & \hspace{4 mm}+Contr. & 1.0 (0.24) & 0.9 (0.2) & 1.4 (0.3) & 1.2 (0.29) & 1.1 (0.38) & 1.6 (0.32) & 1.28 \\ 
 \cmidrule{2-10}
 & \multirow{7}{*}{1k} & PEBBLE & 0.86 (0.15) & 0.53 (0.19) & 0.88 (0.15) & 0.91 (0.14) & 0.73 (0.18) & 0.48 (0.25) & 0.73 \\ 
 &  & \hspace{4 mm}+SimSiam & 1.1 (0.19) & 0.59 (0.14) & 1.2 (0.22) & 1.3 (0.3) & 1.1 (0.21) & 1.0 (0.15) & 1.04 \\ 
 &  & \hspace{4 mm}+Contr. & 1.1 (0.19) & 0.63 (0.16) & 1.2 (0.29) & 1.1 (0.19) & 1.1 (0.19) & 0.83 (0.14) & 0.99 \\ 
 \\
 & & PrefPPO & 0.9 (0.17) & 0.88 (0.17) & 1.1 (0.15) & 0.98 (0.21) & 0.89 (0.18) & 0.83 (0.17) & 0.92 \\ 
 &  & \hspace{4 mm}+SimSiam & 1.2 (0.21) & 0.88 (0.23) & 1.2 (0.27) & 1.2 (0.23) & 1.1 (0.26) & 1.1 (0.16) & 1.11 \\ 
 & & \hspace{4 mm}+Contr. &  1.1 (0.19) & 0.68 (0.28) & 1.2 (0.25) & 1.1 (0.2) & 0.82 (0.31) & 0.56 (0.25) & 0.82 \\ 
 \cmidrule{2-10}
& \multirow{7}{*}{500} & PEBBLE & 0.56 (0.21) & 0.48 (0.21) & 0.66 (0.2) & 0.64 (0.15) & 0.47 (0.22) & 0.48 (0.23) & 0.55 \\ 
 &  & \hspace{4 mm}+SimSiam & 1.1 (0.21) & 0.58 (0.16) & 1.2 (0.24) & 1.0 (0.22) & 1.0 (0.19) & 0.68 (0.16) & 0.93 \\ 
 &  & \hspace{4 mm}+Contr. & 1.1 (0.21) & 0.64 (0.11) & 1.1 (0.22) & 1.1 (0.17) & 1.0 (0.17) & 0.85 (0.14) & 0.97 \\ 
 \\
 & & PrefPPO & 0.8 (0.18) & 0.81 (0.22) & 0.96 (0.12) & 0.72 (0.18) & 0.74 (0.24) & 0.88 (0.17) & 0.82 \\ 
 &  & \hspace{4 mm}+SimSiam & 1.1 (0.2) & 0.76 (0.19) & 1.0 (0.2) & 1.1 (0.25) & 0.89 (0.21) & 0.81 (0.25) & 0.95 \\ 
 & & \hspace{4 mm}+Contr. & 1.1 (0.21) & 0.63 (0.25) & 0.9 (0.28) & 0.89 (0.22) & 0.88 (0.16) & 1.5 (0.48) & 0.95 \\ 
 \cmidrule{2-10}
& \multirow{7}{*}{200} & PEBBLE & 0.54 (0.19) & 0.49 (0.22) & 0.64 (0.15) & 0.46 (0.2) & 0.43 (0.22) & 0.48 (0.23) & 0.51 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.9 (0.17) & 0.57 (0.17) & 0.77 (0.16) & 0.89 (0.14) & 0.76 (0.11) & 0.68 (0.15) & 0.76 \\ 
 &  & \hspace{4 mm}+Contr. & 0.95 (0.15) & 0.53 (0.16) & 0.86 (0.16) & 0.88 (0.14) & 0.77 (0.12) & 0.74 (0.16) & 0.79 \\ 
 \\
 & & PrefPPO & 0.7 (0.23) & 0.59 (0.28) & 0.82 (0.17) & 0.65 (0.27) & 0.8 (0.25) & 0.82 (0.27) & 0.73 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.89 (0.15) & 0.79 (0.23) & 0.95 (0.18) & 0.87 (0.16) & 0.76 (0.26) & 0.79 (0.17) & 0.84 \\ 
 & & \hspace{4 mm}+Contr. & 1.0 (0.33) & 0.7 (0.15) & 0.95 (0.21) & 0.86 (0.18) & 1.2 (0.43) & 1.2 (0.24) & 1.01 \\ 
  \cmidrule{2-10}
& \multirow{7}{*}{100} & PEBBLE & 0.38 (0.21) & 0.47 (0.17) & 0.64 (0.14) & 0.42 (0.22) & 0.46 (0.2) & 0.44 (0.22) & 0.47 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.78 (0.16) & 0.54 (0.2) & 0.98 (0.19) & 0.72 (0.15) & 0.75 (0.16) & 0.67 (0.18) & 0.74 \\ 
 &  & \hspace{4 mm}+Contr. & 0.67 (0.18) & 0.47 (0.2) & 0.89 (0.14) & 0.76 (0.15) & 0.79 (0.17) & 0.65 (0.19) & 0.71 \\ 
 \\
 & & PrefPPO & 0.56 (0.31) & 0.81 (0.31) & 0.66 (0.22) & 0.62 (0.28) & 0.51 (0.31) & 0.6 (0.29) & 0.63 \\ 
 &  & \hspace{4 mm}+SimSiam & 1.0 (0.24) & 0.8 (0.23) & 0.82 (0.19) & 0.71 (0.23) & 0.76 (0.17) & 0.81 (0.26) & 0.82 \\
 & & \hspace{4 mm}+Contr. & 0.91 (0.19) & 0.52 (0.42) & 0.61 (0.32) & 0.6 (0.27) & 0.99 (0.21) & 0.53 (0.37) & 0.69 \\ 
  \cmidrule{2-10}
& \multirow{7}{*}{50} & PEBBLE & 0.38 (0.26) & 0.4 (0.23) & 0.49 (0.2) & 0.42 (0.25) & 0.42 (0.26) & 0.36 (0.26) & 0.41 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.65 (0.16) & 0.47 (0.24) & 0.77 (0.14) & 0.68 (0.18) & 0.67 (0.2) & 0.56 (0.19) & 0.63 \\ 
 &  & \hspace{4 mm}+Contr. & 0.83 (0.12) & 0.49 (0.23) & 0.8 (0.14) & 0.65 (0.18) & 0.69 (0.16) & 0.62 (0.19) & 0.68 \\ 
 \\
 & & PrefPPO & 0.68 (0.3) & 0.64 (0.28) & 0.58 (0.28) & 0.49 (0.26) & 0.49 (0.3) & 0.5 (0.31) & 0.56 \\ 
 &  & \hspace{4 mm}+SimSiam & 0.9 (0.19) & 0.71 (0.29) & 0.9 (0.25) & 0.83 (0.18) & 0.68 (0.26) & 0.77 (0.29) & 0.80 \\ 
 & & \hspace{4 mm}+Contr. & 1.2 (0.34) & 0.58 (0.29) & 0.9 (0.27) & 0.82 (0.16) & 0.47 (0.44) & 1.1 (0.35) & 0.85 \\ 
 \midrule

%% QUADRUPED-RUN RESULTS [NOT INCLUDED IN FINAL VERSION]
% \multicolumn{10}{c}{Quadruped-run}  \\
% \midrule

%  & \multirow{7}{*}{2k} & PEBBLE & 1.0 (0.28) & 0.61 (0.26) & 1.1 (0.3) & 1.2 (0.25) & 1.0 (0.22) & 0.57 (0.26) & 0.91 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.3 (0.48) & 0.68 (0.22) & 1.4 (0.54) & 1.4 (0.55) & 1.3 (0.45) & 1.2 (0.27) & 1.21 \\ 
%  &  & \hspace{4 mm}+Contr. & 1.4 (0.52) & 0.75 (0.2) & 1.4 (0.49) & 1.4 (0.5) & 1.4 (0.6) & 1.0 (0.16) & 1.22 \\ 
%  & & PrefPPO & 1.3 (0.17) & 1.1 (0.19) & 1.5 (0.21) & 1.3 (0.17) & 1.4 (0.21) & 1.3 (0.12) & 1.32 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.4 (0.16) & 1.2 (0.23) & 1.5 (0.17) & 1.2 (0.16) & 1.2 (0.16) & 1.4 (0.17) & 1.32 \\ 
%  & & \hspace{4 mm}+Contr. &  Oracle & Mistake & Equal & Skip & Myopic & Noisy & Mean\\
%  \cmidrule{2-10}
% & \multirow{7}{*}{1k} & PEBBLE & 0.86 (0.21) & 0.52 (0.28) & 1.1 (0.31) & 0.91 (0.21) & 0.88 (0.21) & 0.66 (0.3) & 0.82 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.3 (0.44) & 0.65 (0.2) & 1.3 (0.5) & 1.3 (0.42) & 1.3 (0.41) & 0.96 (0.18) & 1.14 \\ 
%  &  & \hspace{4 mm}+Contr. & 1.2 (0.34) & 0.97 (0.2) & 1.4 (0.57) & 1.2 (0.35) & 1.2 (0.44) & 1.0 (0.16) & 1.17 \\ 
%  & & PrefPPO & 1.1 (0.14) & 1.2 (0.16) & 1.2 (0.15) & 1.1 (0.17) & 1.0 (0.23) & 1.1 (0.14) & 1.11 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.5 (0.18) & 1.3 (0.24) & 1.6 (0.3) & 1.2 (0.2) & 1.5 (0.22) & 1.1 (0.18) & 1.36 \\
%  & & \hspace{4 mm}+Contr. &  Oracle & Mistake & Equal & Skip & Myopic & Noisy & Mean\\
%  \cmidrule{2-10}
% & \multirow{7}{*}{500} & PEBBLE & 0.85 (0.26) & 0.64 (0.25) & 1.2 (0.35) & 0.83 (0.23) & 0.84 (0.26) & 0.68 (0.22) & 0.83 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.3 (0.36) & 0.93 (0.27) & 1.3 (0.5) & 1.2 (0.27) & 1.1 (0.25) & 1.1 (0.21) & 1.15 \\ 
%  &  & \hspace{4 mm}+Contr. & 1.2 (0.38) & 0.98 (0.21) & 1.3 (0.49) & 1.2 (0.33) & 1.2 (0.26) & 1.1 (0.22) & 1.16 \\ 
%  & & PrefPPO & 1.1 (0.14) & 0.95 (0.22) & 1.1 (0.19) & 0.93 (0.26) & 0.83 (0.25) & 1.0 (0.2) & 1.00 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.3 (0.24) & 1.1 (0.18) & 1.2 (0.14) & 1.2 (0.19) & 1.1 (0.18) & 1.4 (0.24) & 1.23 \\ 
%  & & \hspace{4 mm}+Contr. &  Oracle & Mistake & Equal & Skip & Myopic & Noisy & Mean\\
%  \cmidrule{2-10}
% & \multirow{7}{*}{200} & PEBBLE & 0.68 (0.23) & 0.6 (0.25) & 0.78 (0.29) & 0.71 (0.24) & 0.6 (0.24) & 0.64 (0.24) & 0.67 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.1 (0.24) & 0.65 (0.19) & 1.2 (0.34) & 1.1 (0.26) & 1.1 (0.23) & 0.83 (0.19) & 0.98 \\ 
%  &  & \hspace{4 mm}+Contr. & 1.1 (0.34) & 0.73 (0.2) & 1.2 (0.37) & 1.2 (0.26) & 1.2 (0.32) & 0.91 (0.14) & 1.05 \\ 
%  & & PrefPPO & 0.86 (0.29) & 0.83 (0.35) & 0.83 (0.2) & 0.78 (0.29) & 0.87 (0.29) & 0.86 (0.27) & 0.84 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.3 (0.14) & 1.1 (0.31) & 1.4 (0.2) & 1.4 (0.15) & 1.2 (0.18) & 1.2 (0.14) & 1.27 \\
%  & & \hspace{4 mm}+Contr. &  Oracle & Mistake & Equal & Skip & Myopic & Noisy & Mean\\
%  \cmidrule{2-10}
% & \multirow{7}{*}{100} & PEBBLE & 0.55 (0.25) & 0.57 (0.23) & 0.68 (0.27) & 0.71 (0.21) & 0.55 (0.26) & 0.64 (0.24) & 0.62 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.1 (0.23) & 0.68 (0.19) & 1.1 (0.36) & 1.0 (0.21) & 0.99 (0.18) & 1.0 (0.3) & 0.98 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.96 (0.19) & 0.72 (0.24) & 1.0 (0.22) & 1.1 (0.21) & 1.0 (0.25) & 0.97 (0.23) & 0.96 \\ 
%  & & PrefPPO & 0.69 (0.25) & 0.87 (0.31) & 0.91 (0.21) & 0.79 (0.31) & 0.77 (0.27) & 0.87 (0.29) & 0.82 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.0 (0.14) & 1.2 (0.25) & 1.1 (0.24) & 1.3 (0.21) & 0.98 (0.22) & 0.99 (0.25) & 1.10 \\ 
%  & & \hspace{4 mm}+Contr. &  Oracle & Mistake & Equal & Skip & Myopic & Noisy & Mean\\
% & \multirow{7}{*}{50} & PEBBLE & 0.58 (0.25) & 0.56 (0.25) & 0.62 (0.23) & 0.59 (0.25) & 0.62 (0.24) & 0.53 (0.28) & 0.58 \\ 
%  &  & \hspace{4 mm}+SimSiam & 0.91 (0.22) & 0.71 (0.19) & 0.96 (0.22) & 0.96 (0.31) & 0.8 (0.23) & 0.78 (0.17) & 0.85 \\ 
%  &  & \hspace{4 mm}+Contr. & 0.74 (0.18) & 0.76 (0.19) & 1.0 (0.24) & 0.8 (0.18) & 0.96 (0.21) & 0.75 (0.24) & 0.84 \\ 
%  & & PrefPPO & 0.77 (0.3) & 0.72 (0.33) & 0.78 (0.32) & 0.79 (0.33) & 0.72 (0.25) & 0.75 (0.31) & 0.76 \\ 
%  &  & \hspace{4 mm}+SimSiam & 1.1 (0.19) & 1.1 (0.28) & 1.2 (0.26) & 1.3 (0.2) & 0.88 (0.25) & 1.1 (0.24) & 1.11 \\ 
%  & & \hspace{4 mm}+Contr. &  Oracle & Mistake & Equal & Skip & Myopic & Noisy & Mean\\
%  \midrule

%% BUTTON-PRESS RESULTS
\multicolumn{10}{c}{Button-Press}  \\
\midrule
  & \multirow{5}{*}{20k} & PEBBLE & 0.72 (0.26) & 0.57 (0.26) & 0.77 (0.25) & 0.75 (0.26) & 0.68 (0.21) & 0.72 (0.24) & 0.70 \\ 
 &  & \hspace{4 mm}+Contr. & 0.65 (0.25) & 0.61 (0.28) & 0.67 (0.27) & 0.67 (0.27) & 0.67 (0.24) & 0.69 (0.26) & 0.66 \\ 
 \\
 &  & PrefPPO & 0.18 (0.03) & 0.18 (0.04) & 0.21 (0.03) & 0.18 (0.03) & 0.17 (0.04) & 0.17 (0.04) & 0.18 \\ 
 &  & \hspace{4 mm}+Contr. & 0.22 (0.03) & 0.17 (0.03) & 0.22 (0.02) & 0.17 (0.03) & 0.19 (0.03) & 0.17 (0.04) & 0.19 \\
 \cmidrule{2-10}
 & \multirow{5}{*}{10k} & PEBBLE & 0.66 (0.26) & 0.47 (0.21) & 0.67 (0.27) & 0.63 (0.26) & 0.67 (0.24) & 0.6 (0.26) & 0.62 \\ 
 &  & \hspace{4 mm}+Contr. & 0.65 (0.27) & 0.61 (0.3) & 0.66 (0.27) & 0.62 (0.26) & 0.6 (0.25) & 0.68 (0.28) & 0.64 \\
 \\
 &  & PrefPPO & 0.18 (0.03) & 0.14 (0.04) & 0.19 (0.03) & 0.17 (0.04) & 0.18 (0.03) & 0.17 (0.04) & 0.17 \\ 
 &  & \hspace{4 mm}+Contr. & 0.15 (0.04) & 0.12 (0.05) & 0.18 (0.03) & 0.17 (0.03) & 0.17 (0.03) & 0.16 (0.03) & 0.16 \\ 
 \cmidrule{2-10}
& \multirow{5}{*}{5k} & PEBBLE & 0.48 (0.21) & 0.31 (0.12) & 0.56 (0.25) & 0.54 (0.24) & 0.59 (0.23) & 0.52 (0.23) & 0.50 \\ 
 &  & \hspace{4 mm}+Contr. & 0.55 (0.24) & 0.54 (0.26) & 0.65 (0.27) & 0.63 (0.26) & 0.57 (0.24) & 0.63 (0.28) & 0.60 \\ 
 \\
 &  & PrefPPO & 0.15 (0.04) & 0.13 (0.05) & 0.19 (0.03) & 0.16 (0.04) & 0.16 (0.04) & 0.14 (0.04) & 0.15 \\ 
 &  & \hspace{4 mm}+Contr. & 0.14 (0.04) & 0.13 (0.05) & 0.18 (0.03) & 0.14 (0.04) & 0.14 (0.04) & 0.14 (0.03) & 0.14 \\ 
 \cmidrule{2-10}
& \multirow{5}{*}{2.5k} & PEBBLE & 0.37 (0.18) & 0.21 (0.088) & 0.44 (0.21) & 0.34 (0.15) & 0.4 (0.17) & 0.34 (0.18) & 0.35 \\ 
 &  & \hspace{4 mm}+Contr. & 0.49 (0.25) & 0.42 (0.22) & 0.52 (0.24) & 0.5 (0.23) & 0.44 (0.17) & 0.45 (0.21) & 0.47 \\ 
 \\
 &  & PrefPPO & 0.14 (0.04) & 0.12 (0.05) & 0.13 (0.05) & 0.13 (0.05) & 0.13 (0.05) & 0.14 (0.05) & 0.13 \\ 
 &  & \hspace{4 mm}+Contr. & 0.14 (0.04) & 0.11 (0.05) & 0.15 (0.04) & 0.11 (0.04) & 0.14 (0.04) & 0.13 (0.04) & 0.13 \\  
\midrule

%% SWEEP INTO RESULTS
\multicolumn{10}{c}{Sweep-into}  \\
\midrule

 & \multirow{5}{*}{20k} & PEBBLE & 0.53 (0.25) & 0.26 (0.15) & 0.51 (0.23) & 0.52 (0.27) & 0.47 (0.28) & 0.47 (0.26) & 0.46 \\ 
 &  & \hspace{4 mm}+Contr. & 0.5 (0.22) & 0.36 (0.13) & 0.41 (0.2) & 0.6 (0.22) & 0.54 (0.21) & 0.61 (0.25) & 0.50 \\ 
 \\
 & & PrefPPO & 0.16 (0.046) & 0.14 (0.047) & 0.16 (0.069) & 0.18 (0.065) & 0.19 (0.063) & 0.08 (0.026) & 0.15 \\ 
 &  & \hspace{4 mm}+Contr. & 0.23 (0.064) & 0.11 (0.042) & 0.2 (0.058) & 0.2 (0.051) & 0.19 (0.054) & 0.1 (0.034) & 0.17 \\ 
 \cmidrule{2-10}
 & \multirow{5}{*}{10k} & PEBBLE & 0.28 (0.12) & 0.22 (0.13) & 0.45 (0.21) & 0.33 (0.17) & 0.47 (0.25) & 0.51 (0.24) & 0.38 \\ 
 &  & \hspace{4 mm}+Contr. & 0.47 (0.23) & 0.3 (0.14) & 0.45 (0.24) & 0.32 (0.21) & 0.42 (0.22) & 0.44 (0.21) & 0.40 \\ 
 \\
 & & PrefPPO & 0.16 (0.048) & 0.19 (0.064) & 0.18 (0.05) & 0.18 (0.049) & 0.12 (0.055) & 0.058 (0.024) & 0.15 \\ 
 &  & \hspace{4 mm}+Contr. & 0.11 (0.034) & 0.12 (0.046) & 0.15 (0.046) & 0.16 (0.056) & 0.11 (0.052) & 0.054 (0.029) & 0.12 \\ 
 \cmidrule{2-10}
& \multirow{5}{*}{5k} & PEBBLE & 0.17 (0.099) & 0.17 (0.089) & 0.28 (0.19) & 0.24 (0.15) & 0.23 (0.13) & 0.22 (0.12) & 0.22 \\ 
 &  & \hspace{4 mm}+Contr. & 0.34 (0.14) & 0.23 (0.19) & 0.52 (0.24) & 0.37 (0.2) & 0.4 (0.24) & 0.44 (0.18) & 0.38 \\ 
 \\
 & & PrefPPO & 0.1 (0.039) & 0.078 (0.027) & 0.1 (0.032) & 0.092 (0.025) & 0.1 (0.038) & 0.051 (0.019) & 0.09 \\ 
 &  & \hspace{4 mm}+Contr. & 0.14 (0.052) & 0.097 (0.034) & 0.12 (0.032) & 0.14 (0.076) & 0.1 (0.026) & 0.043 (0.026) & 0.11 \\ 
 \cmidrule{2-10}
& 2.5k & PEBBLE & 0.15 (0.086) & 0.13 (0.076) & 0.16 (0.1) & 0.16 (0.088) & 0.18 (0.075) & 0.25 (0.11) & 0.17 \\ 
 & \multirow{4}{*}{2.5k} & \hspace{4 mm}+Contr. & 0.21 (0.13) & 0.19 (0.22) & 0.29 (0.17) & 0.17 (0.092) & 0.25 (0.15) & 0.28 (0.16) & 0.23 \\ 
 \\
 & & PrefPPO & 0.092 (0.032) & 0.097 (0.044) & 0.15 (0.051) & 0.15 (0.049) & 0.099 (0.035) & 0.032 (0.022) & 0.10 \\ 
 &  & \hspace{4 mm}+Contr. & 0.058 (0.019) & 0.048 (0.018) & 0.11 (0.032) & 0.072 (0.035) & 0.07 (0.016) & 0.036 (0.017) & 0.07 \\ 
 
\end{longtable}
\end{sc}
\end{scriptsize}
\end{center}
\end{landscape}
